ENDF/B-VIII.1: Updated Nuclear Reaction Data Library for Science and Applications

The ENDF/B-VIII.1 library is the newest recommended evaluated nuclear data file by the Cross Section Evaluation Working Group (CSEWG) for use in nuclear science and technology applications, and incorporates advances made in the six years since the release of ENDF/B-VIII.0. Among key advances made are that the $^{239}$Pu file was reevaluated by a joint international effort and that updated $^{16,18}$O, $^{19}$F, $^{28-30}$Si, $^{50-54}$Cr, $^{55}$Mn, $^{54,56,57}$Fe, $^{63,65}$Cu, $^{139}$La, $^{233,235,238}$U, and $^{240,241}$Pu neutron nuclear data from the IAEA coordinated INDEN collaboration were adopted. Over 60 neutron dosimetry cross sections were adopted from the IAEA's IRDFF-II library. In addition, the new library includes significant changes for $^3$He, $^6$Li,$^9$Be, $^{51}$V, $^{88}$Sr, $^{103}$Rh, $^{140,142}$Ce, Dy, $^{181}$Ta, Pt, $^{206-208}$Pb, and $^{234,236}$U neutron data, and new nuclear data for the photonuclear, charged-particle and atomic sublibraries. Numerous thermal neutron scattering kernels were reevaluated or provided for the very first time. On the covariance side, work was undertaken to introduce better uncertainty quantification standards and testing for nuclear data covariances. The significant effort to reevaluate important nuclides has reduced bias in the simulations of many integral experiments with particular progress noted for fluorine, copper, and stainless steel containing benchmarks. Data issues hindered the successful deployment of the previous ENDF/B-VIII.0 for commercial nuclear power applications in high burnup situations. These issues were addressed by improving the $^{238}$U and $^{239,240,241}$Pu evaluated data in the resonance region. The new library performance as a function of burnup is similar to the reference ENDF/B-VII.1 library. The ENDF/B-VIII.1 data are available in ENDF-6 and GNDS format at https://doi.org/10.11578/endf/2571019.

==> fpy/nfy.tex <==
%!TEX root = endf-VIII-1.tex

%
\fixme{ Text on updates on neutron induced fission yields. }

\begin{itemize}

\item \nuc{227}{Th}
\item \nuc{229}{Th}
\item \nuc{232}{Th}
\item \nuc{231}{Pa}
\item \nuc{232}{U}
\item \nuc{233}{U}
\item \nuc{234}{U}
\item \nuc{235}{U}
\item \nuc{236}{U}
\item \nuc{237}{U}
\item \nuc{238}{U}
\item \nuc{237}{Np}
\item \nuc{238}{Np}
\item \nuc{238}{Pu}
\item \nuc{239}{Pu}
\item \nuc{240}{Pu}
\item \nuc{241}{Pu}
\item \nuc{242}{Pu}
\item \nuc{241}{Am}
\item \nuc{242m1}{Am}
\item \nuc{243}{Am}
\item \nuc{242}{Cm}
\item \nuc{243}{Cm}
\item \nuc{244}{Cm}
\item \nuc{245}{Cm}
\item \nuc{246}{Cm}
\item \nuc{248}{Cm}
\item \nuc{249}{Cf}
\item \nuc{251}{Cf}
\item \nuc{254}{Es}
\item \nuc{255}{Fm}

\end{itemize}



==> fpy/sfy.tex <==
%!TEX root = endf-VIII-1.tex


\fixme{ Text on updates on spontaneous fission yields.  }

\begin{itemize}

\item \nuc{238}{U} 
\item \nuc{244}{Cm}
\item \nuc{246}{Cm}
\item \nuc{248}{Cm}
\item \nuc{250}{Cf}
\item \nuc{252}{Cf}
\item \nuc{253}{Es}
\item \nuc{254}{Fm}
\item \nuc{256}{Fm}

\end{itemize}


